On how to avoid exacerbating spurious correlations when models are overparameterized

Overparameterized models fail to generalize well in the presence of data imbalance even when combined with traditional techniques for mitigating imbalances. This paper focuses on imbalanced classification datasets, in which a small subset of the population -- a minority -- may contain features that correlate spuriously with the class label. For a parametric family of cross-entropy loss modifications and a representative Gaussian mixture model, we derive non-asymptotic generalization bounds on the worst-group error that shed light on the role of different hyper-parameters. Specifically, we prove that, when appropriately tuned, the recently proposed VS-loss learns a model that is fair towards minorities even when spurious features are strong. On the other hand, alternative heuristics, such as the weighted CE and the LA-loss, can fail dramatically. Compared to previous works, our bounds hold for more general models, they are non-asymptotic, and, they apply even at scenarios of extreme imbalance.

==> LAloss.tex <==


%\section{LA}
%% ----------------------------
\subsection{\red{Theorem \ref{thm:LALoss}}}
In this section we provide proof of Theroem \ref{thm:LALoss} and the relevant lemmas. Through out this section, we assume $\Delta_\pm=1$, consequently $\ell_{i,t} = \omega_{g_i}e^{-y_i\,\inp{\x_i}{\w^{t}}+\iota_{g_i}}$, and $\ellp_{i,t}=\ell_{i,t}$.

%\begin{theorem}\label{thm:LALoss}
%	Under the assumptions of Theorem \ref{thm:main}, the worst-group test error achieved by gradient descent iterates on $\ell_{\text{exp, LA}}$ as $t\rightarrow\infty$ is bounded below by
%	
%	\begin{align}
%	\Rc_{wst}^\infty\geq Q(\frac{c\sqrt{n}}{\sqrt{d}}(\frac{R_-}{R_+}+\frac{1}{\tau})R_+),
%	\end{align}
%	where $Q$ is the Q-function.\\
%	
%	
%\end{theorem}


\begin{lemma}\label{lem:ratio2}
	When a good event $\Ec$ holds, with sufficiently small step size, the following inequality is satisfied for all GD steps of LA-loss,
	\begin{align}
	\max_{i,j\in[n]}\Big\{\frac{\ellp_{i,t}}{\ellp_{j,t}}\Big\}\leq c_2
	\end{align} 
	where 
	\begin{align}
	c_2 = \max \{4c_1^2, \frac{\omega_+ e^{\iota_+}}{\omega_- e^{\iota_-}}, \frac{\omega_- e^{\iota_-}}{\omega_+ e^{\iota_+}}\}	\label{eq:lossratio_cond}
	\end{align}
\end{lemma}
Note again that LA-loss is equivalent to VS-loss when $\Delta_\pm=1$. Following the steps in the proof of Lemma \ref{lem:key}, we can prove this statement similarly.	\eqref{eq:lossratio_cond} is to make sure the base case of the induction is satisfied.



\begin{lemma}
	Assuming we have a realization of a good event $\Ec$, for iteration $t$ and $b \in \{\pm 1\}$, let $\rho_{t,b}$ and $\Lpt$ defined as in Lemma \ref{lem:corrLB}, and denote $L^\prime_t = \Lpt + \Lptneg$. Then, there exist $t_0>0$ and $c', c''>0$ such that for all iteration $t>t_0$ and any group $b$,
	\begin{align}
	\rho_{t+1,b} &\leq \rho_{t_0,b} + \eta c' R_+ \Big(\frac{n_b}{n_{-b}} + \frac{R_-}{R_+} + c_1\sqrt{\frac{\log(n/\delta)}{R_+}}\Big) L^\prime_t \label{eq:corrtheorem2}\\
	\|\w^{t}\|_2 &\geq \|\w^{t_0}\|_2+\eta c''\sqrt{\frac{d}{n}}L^\prime_t \label{eq:normtheorem2}
	\end{align}
\end{lemma}
\begin{proof}
	By the application of gradient descent steps and equations \eqref{eq:zmu_same} and \eqref{eq:zmu_same_sharp},
	\begin{align*}
	\rho_{t+1,b} &- \rho_{t,b} \leq \eta \Big[\sum_{i\in\Tc_{b}} \ellp_{i,t} \inp{\z_i}{\nub_b}
	+ \sum_{i\in\Tc_{-b}} \ellp_{i,t} \inp{\z_i}{\nub_b}
	\Big]\\
	&\leq c_2\eta\Big[\frac{3R_+}{2} \frac{n_b}{n} + (R_-+c_1\sqrt{R_+ \log(n/\delta)}) \frac{n_{-b}}{n} \Big] L^\prime _t\\
	&\leq \eta c^\prime R_+ \Big[\frac{n_b}{n_{-b}} + \frac{R_-}{R_+} + c_1\sqrt{\frac{\log(n/\delta)}{R_+}} \Big] L^\prime _t
	\end{align*}
	where in the second line we use Lemma \ref{lem:ratio2}. By repeating this inequality, equation \eqref{eq:corrtheorem2} is proven.
	
	\red{
		The second statement follows similar to Lemma C.2 in [??], by applying GD step and Lemma \ref{lem:maxmarg}.}
	\\
	\tina{The following proof can be omitted and replaced by the red part above!}\\
	For the second statement, from the gradient descent iteration:
	\begin{align}
	\|\w^{t+1}\|_2^2 &= \|\w^{t} + \eta\sum_{i=1}^n \ellp_{i,t} \z_i\|_2^2 \nonumber\\
	&\geq \|\w^{t}\|_2^2  + 2\eta\sum_{i=1}^n \ellp_{i,t} \inp{\z_i}{\w^t} \label{eq:norm}
	\end{align}
	
	Based on Lemma \ref{lem:maxmarg}, the data is linearly separable. [??] proved that gradient descent iterates on a family of loss functions, including exponential and logistic function, will converge in direction to the max margin solution, provided that the data is separable, and the step size is small enough. Thus, for large $t$:
	
	\begin{align}
	\inp{\z_i}{\frac{\w^t}{\|\w^t\|_2}} \geq \frac{c'''}{2} \sqrt{\frac{d}{n}} \label{eq:GDmargin}
	\end{align}
	
	Combining equations \eqref{eq:norm} and \eqref{eq:lbcorr},
	\begin{align*}
	\|\w^{t+1}\|^2_2 &\geq \|\w^{t}\|^2_2 \bigg[1 + \frac{\eta c'''\sqrt{\frac{d}{n}} L^\prime_t}{\|\w^t\|_2}\bigg]
	\end{align*}
	
	
	[??] further show that the loss function at GD steps will be decreasing during training, and as $t$ increases, $\norm{\w^t}_2$ gets to $\infty$. Therefore, as $\norm{\w^0}_2 = 0$, $L^\prime_t \leq \sum_{i=0}^n \omega_{g_i}e^{\iota_{g_i}}$, and after a point in the training, 
	\begin{align}\label{eq:GDnorm}
	\norm{\w^t}_2 \geq \frac{\eta c''' \sqrt{\frac{d}{n}}	\sum_{i=0}^n \omega_{g_i}e^{\iota_{g_i}}}{8}
	\end{align}
	
	Assuming that $t_0$ is large enough to satisfy both \eqref{eq:GDmargin} and \eqref{eq:GDnorm}, for $t>t_0$ we have, 
	\begin{align*}
	\|\w^{t+1}\|_2 &\geq \|\w^{t}\|_2 + \eta c''\sqrt{\frac{d}{n}} \sum_{i=1}^n L^\prime_t
	\end{align*}
	Finally, \eqref{eq:normtheorem2} follows by repeatedly applying this inequality.\\
	
\end{proof}

\subsection{Proof of Theorem \ref{thm:LALoss}}
Putting \eqref{eq:corrtheorem2} and \eqref{eq:normtheorem2} together for $t>t_0$,
\begin{align*}
\frac{\rho_{t,b}}{\|\w^t\|_2} &\leq \frac{\rho_{t_0,b} + \eta c' R_+ \big(\frac{n_b}{n_{-b}} + \frac{R_-}{R_+} + c_1\sqrt{\frac{\log(n/\delta)}{R_+}}\big) L^\prime_{t_0:t}}{\|\w^{t_0}\|_2+\eta c''\sqrt{\frac{d}{n}} L^\prime_{t_0:t}}
%&= c\sqrt{\frac{n}{d}}R_+(\frac{R_-}{R_+} + \frac{n_b}{n_{-b}}).	
\end{align*}
From GD step and \eqref{eq:z_norm}, we have $\norm{\w^t}_2 \leq \norm{\w^{t_0}}_2 + \eta L^\prime_{t_0:t} $. Since $\norm{\w^t}_2$ \red{may need ref and explanatino} is unbounded, we can conclude that $L^\prime_{t_0:t} \rightarrow \infty$ as $t$ gets large. Hence, the second term containing $L^\prime_{t_0:t}$ will dominate and for large $t$,
\begin{align}
\lim_{t\to\infty} \frac{\inp{\w^t}{\nub_{b}}}{\|\w^t\|_2} &\leq cR_+\sqrt{\frac{n}{d}}\Big( \frac{n_b}{n_{-b}} + \frac{R_-}{R_+} + c_1\sqrt{\frac{\log(n/\delta)}{R_+}} \Big).
\end{align}
We assumed that group $b=-1$ is the minority group. Thus, the term above is minimized when $b=-1$. Finally, the worst-group error can be bounded as follows.
\begin{align*}
\Rc_{wst, \rm{LA}}^\infty &=Q\big(\min_{b\in\{\pm 1\}}\inp{\nicefrac{\w^\infty}{\|\w^\infty\|_2}}{{\nub_{b}}}\big)\\
&\geq Q\Bigg(c\,R_+\,\sqrt{\frac{n}{d}}\,\Big(\frac{1}{\tau} + \frac{R_-}{R_+}+ 
{c_1\sqrt{\frac{\log(n/\delta)}{R_+}}} \Big)\Bigg).
\end{align*}

\tina{ref to importance weight paper or GD follows reg. path}





==> app.tex <==
%\ct{The $C$ in the statements below should be interpreted as ``for all large $C$"}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}[Good event $\Ec$]\label{lem:good}
 Further letting Assumption \ref{ass:dim} hold for $C>0$ and $\delta$, there exists constant $c>1$ such that with probability $1-\delta$ over the realization of the training set the data are linearly separable and the following events hold simultaneously for $b\in\{\pm1\}$,
\begin{align}
%&\forall i\in\Tc_{b}\,:\,|\z_i^T\nub_b - R_+|\leq  R_+/2
%\label{eq:zmu_same}
%\\
&{\forall i\in\Tc_{b}\,:\, |\z_i^T\nub_{\pm b}- R_{\pm}| \leq c_1\sqrt{R_+}\sqrt{\log(n/\delta)}
\label{eq:zmu_same_sharp_app}}
%\\
%&\forall i\in\Tc_{b}\,:\,|\z_i^T\nub_{-b}-  R_-| \leq c_1\sqrt{R_+}\sqrt{\log(n/\delta)}
%\label{eq:zmu_diff}
%\\
%&\forall i\in[n]\,:\,d/c_1 \leq \|\z_i\|_2^2\leq c_1d
%\label{eq:z_norm2}
\\
&{\forall i\in[n]\,: \|\z_i\|_2 \leq c_1(\sqrt{R_+} + \sqrt{d})} 
\label{eq:z_norm_app}
\\
&{\forall i\in[n]\,: \|\z_i\|_2 \geq \begin{cases}
(\sqrt{R_+}/c_1 -  \sqrt{d}) & R_+>c_1^2{d},\\
(\sqrt{d}/c_1 -  \sqrt{R_+}) & d>c_1^2{R_+}\\
\end{cases}
}
\label{eq:z_norm_lb_app}
\\
%\\
%&\red{\forall i\in[n]\,: |\|\z_i\|_2 - \sqrt{R_+}| \leq c_1\sqrt{d\log(n/\delta)} }
%\label{eq:z_norm}
%\\
%&\forall i\in\Tc_{b}, j\in\Tc_{-b}\,:|\z_i^T\z_j - R_-| \leq c_1\big(\sqrt{R_+}+\sqrt{d}\big) \sqrt{\log(n/\delta)}
%\label{eq:z_ortho}
%\\
&\forall \Tc_{b}\ni i\neq j\in\Tc_{\pm b}\,:|\z_i^T\z_j - {R_\pm}| \leq c_1\big(\sqrt{R_+}+\sqrt{d}\big) \sqrt{\log(n/\delta)}
\label{eq:z_align_app}
\end{align}
When all the above holds, we say that good event $\Ec$ holds.
\end{lemma}




%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{lemma}[Data separability and max-margin]\label{lem:maxmarg}
For any $\delta\in(0,1)$, there exists large enough constants $C_i>0$ such that with probability at least $1-\delta$ the training data are linearly separable, provided that $d\geq C_1\|\mub_c\|_2^2 n$, $\|\mub_c\|_2\geq C_2\sqrt{\log(n/\delta)}$ and $n\geq C_3$. Moreover, under the same conditions, with probability $1-\delta$ the maximum margin is lower bounded as follows for some constant $c>0$:
\begin{align}
\max_{\|\w\|=1}\min_{i\in[n]} \inp{\w}{\z_i} \geq c'''\sqrt{\frac{d}{n}}\,.
\end{align}
\end{lemma}

\begin{proof}
Recall the notation following notation for $i\in[n]$:
$$
\z_i:=\begin{bmatrix}
\z_{i,c} \\
\z_{i,s}
\end{bmatrix} := y_i\begin{bmatrix}
\x_{i,c} \\
\x_{i,s}
\end{bmatrix} = \begin{bmatrix}
\mub_c + \q_{i,c}\\
(y_ia_i)\,\mub_s + \q_{i,s}
\end{bmatrix} 
$$
where $\q_{i,c},\q_{i,s}\sim\Nn(0,I_d)$  and independent of each other. We will prove that 
$$
\wt:= \sum_{i\in[n]}\begin{bmatrix}
\z_{i,c} \\
0
\end{bmatrix}
$$
is a linear separator under the lemma's assumptions.
Indeed, we have for any $j\in[n]$:
\begin{align}
\inp{\wt}{\z_j} = \|\z_{j,c}\|^2 + \inp{\z_{j,c}}{\sum_{j\neq i}\z_{i,c}}.
\end{align}
In the sequel, $c_1>1$ is a constant. First, with probability at least $1-\delta/2$ it holds simultaneously for all $j\in[n]$ that:
\begin{subequations}\label{eq:event_sep}
\begin{align}
%\|\z_{j,c}\| &\geq \|\mub_c\| - c_1\sqrt{d \log(n/\delta)},\\
&d/c_1 \leq \|\z_{j,c}\|^2 \leq c_1 d,\\
&\inp{\z_{j,c}}{\mub_c}\leq \|\mub_c\|_2^2 + c_1\|\mub_c\|\sqrt{\log(n/\delta)}.
\end{align}
\end{subequations}
Above, the first inequality holds because for large enough $C$, by assumption $d>C\|\mub\|_2^2$ and $\log(n/\delta)\geq C$.
Second, since $\z_{i,c}, i\in[n]$ are i.i.d, we have that $\sum_{j\neq i}\z_{i,c}\sim\Nn((n-1)\mub_c,\sqrt{n}I_d)$ and is independent of $\z_{j,c}.$ Hence, conditioned on $\z_{j,c}$:
$$
\inp{\z_{j,c}}{\sum_{j\neq i}\z_{i,c}} \stackrel{(P)}{=}(n-1)\inp{\z_{j,c}}{\mub_c} + \| \z_{j,c}\|_2 \sqrt{n-1}\cdot G_j,\text{ with } G_j\sim\Nn(0,1).
$$
Thus, in the event \eqref{eq:event_sep}, with probability $1-\delta/2$, simultaneously for all $j\in[n]$:
$$
\inp{\z_{j,c}}{\sum_{j\neq i}\z_{i,c}}\leq n\|\mub_c\|_2^2 + c_1\|\mub_c\|n\sqrt{\log(n/\delta)}+c_1\sqrt{d n}\sqrt{\log(n/\delta)}.
$$
Putting things together, with probability at least $1-\delta$, simultaneously for all $j\in[n]$, it holds that
\begin{align*}
&\frac{1}{n}\inp{\wt}{\z_j} \geq \frac{d}{c_1 n} 
\\ &\quad-\Big(\|\mub_c\|^2 + c_1\|\mub_c\|\sqrt{\log(n/\delta)}+c_1\sqrt{\frac{d{\log(n/\delta)}}{n}}\Big)
\end{align*}
By invoking $\sqrt{\log(n/\delta)}\leq \|\mub_c\|/C_2$ for some constant $C_2>0$ and picking large enough $C_1$ such that $d/n\geq C_1 \|\mub_c\|^2$, this shows that for some $c'>1$:
\begin{align}\label{eq:inp_bound_sep}
\min_{i\in[n]} \inp{\wt}{\z_i} \geq d/c' >0.
\end{align}
Therefore, the $\wt$ is a linear separator. 

Next, we upper bound the norm of $\wt$. With probability $1-\delta$:
\begin{align}
\|\wt\|_2 = \| n\mub_c + \sum_{i\in[n]}\q_{i,c}\| \leq n\|\mub_c\| + c_1\sqrt{n}\sqrt{d}
\end{align}
where the upper bound follows by triangle inequality and using that $\sum_{i\in[n]}\q_{i,c}\sim\Nn(0,\sqrt{n} I_d)$ to invoke Fact \ref{fact:g_norm}. Under the conditions of the lemma, $\|\mub_c\|\sqrt{n}\leq \sqrt{d}/\sqrt{C_1}$ . Hence,  for some $c''\geq 1$:
\begin{align}\label{eq:norm_bound_sep}
\|\wt\|_2  \leq c'' \sqrt{n}\sqrt{d}.
\end{align}

Putting together \eqref{eq:inp_bound_sep} and \eqref{eq:norm_bound_sep}, we conclude with the second statement of the lemma, i.e.
$$
\max_{\|\w\|=1}\min_{i\in[n]} \inp{\w}{\z_i}  \geq \frac{\min_{i\in[n]}\inp{\wt}{\z_j}}{\|\wt\|_2} \geq c'''\sqrt{\frac{d}{n}}\,.
$$
  
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}
Let $n>1$ training data under Assumption \ref{ass:means}. For any $\delta\in(0,1)$, there exists $c>1$ such that with probability $1-\delta$ the following statements are true simultaneously for all $i\in[n]$:
\begin{align}
\|\z_i\|_2 \leq \sqrt{d} + \sqrt{R_+} + c\sqrt{\log(n/\delta)}
\end{align}
and
\begin{align}
\|\z_i\|_2 \geq \begin{cases}
\sqrt{R_+}-\sqrt{d} - c\sqrt{\log(n/\delta)}, & R_+>\sqrt{d}\\
\sqrt{d}-\sqrt{R_+} - c\sqrt{\log(n/\delta)}, & R_+<\sqrt{d}
\end{cases}
\end{align}
Further assuming $\min\{d,R_+\}\geq C{\log(n/\delta)}$ for a large enough constant $C>0$, there exists constant $c>1$ such that
\begin{align}
\|\z_i\|_2^2 \leq c(\sqrt{d} + \sqrt{R_+})^2
\end{align}
and
\begin{align}
\|\z_i\|_2^2 \geq \begin{cases}
(\sqrt{R_+}/c-\sqrt{d})^2, & R_+>c\sqrt{d}\\
(\sqrt{d}/c-\sqrt{R_+})^2, & cR_+<\sqrt{d}
\end{cases}
\end{align}
\end{lemma}

\begin{proof}
By Fact \ref{fact:g_norm} and union bound, with probability at least $1-\delta$:
$$
\forall i\in[n]: |\|\z_i-\nub_i\|_2-\sqrt{d}|\leq c\sqrt{\log(n/\delta)}.
$$
Recall that $\|\nub_i\|_2=\sqrt{R_+}$ for all $i\in[n]$. Hence, the desired follows from the above and triangle inequality. 
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}
For any $\delta\in(0,1)$, there exists large enough constants $C_i>0$ such that with probability at least $1-\delta$ over the training data, the following inequalities hold simultaneously for $b\in\{\pm1\}$, provided that $d\geq C_1\|\mub_c\|_2^2 n$, $\|\mub_c\|_2\geq C_2\sqrt{\log(n/\delta)}$ and $n\geq C_3$.
\begin{align}
\forall i\in\Tc_{b}: \sum_{\substack{j\in \Tc_b\\j\neq i}}\inp{\z_i}{\z_j} 
\end{align}
\end{lemma}

\begin{proof}
Fix $i\in\Tc_b$ and denote $\z_{-i}:= \sum_{\substack{j\in \Tc_b\\j\neq i}}\z_j.$ Notice that
$\z_{-i}\sim\Nn\big((n_b-1)\nub_b,({n_b-1})I_d\big)$ and is independent of $\z_i$. Thus, conditioned on $\z_i$, we have that
$$
\inp{\z_i}{\z_{-i}} \sim \Nn\big((n_b-1)\inp{\nub_b}{\z_i},\|\z_i\|^2({n_b-1})\big).
$$
Moreover, with probability $1-\frac{\delta}{8n}$ for some constant $c_1\geq 1$:
\begin{align}
%\|\z_{j,c}\| &\geq \|\mub_c\| - c_1\sqrt{d \log(n/\delta)},\\
&\dR/c_1 \leq \|\z_{i}\| \leq c_1 \dR,\\
&|\inp{\z_{i}}{\nub_b}- R_+| \leq c_1\sqrt{R_+}\sqrt{\log(n/\delta)} \leq R_+/2,
\end{align}
where in the last inequality we used that $R_+\geq C\sqrt{\log(n/\delta)}$ for large $C$. Putting things together, with probability $1-\frac{\delta}{4n}$:
\begin{align*}
&\frac{n_bR_+}{c_1} - c_1\sqrt{n\dR\log(n/\delta)}\leq \inp{\z_i}{\z_{-i}}  
\\
&\qquad\qquad\leq c_1n_bR_+ + c_1\sqrt{n\dR\log(n/\delta)}.
\end{align*}
Taking a union bound over all $i\in[n]$ shows \eqref{eq:}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Useful Facts}
\begin{fact}\label{fact:g_norm}
Let $\g\in\R^d$ have entries i.i.d $\Nn(0,1)$. 
Then,
$$
\Pro\left(\|\g\|_2>t\right)\leq 2e^{-t^2/2}.
$$
Specifically, for fixed  $\delta$ such that for some constant $C>0$ it holds $d>C\log(1/\delta)$, there exists $c\geq 1$ such that with probability at least $1-\delta$,
$$
\sqrt{d}/ c \leq  \|\g\|_2 \leq c \sqrt{d}.
$$
\end{fact}




==> proofs.tex <==

%\ct{If needed add a Table for notations. Too much :)}
This section includes the proof of Theorem \ref{thm:main}. Without further explicit reference, we assume $n$ training data generated as in Assumption \ref{ass:means}. For convenience, we introduce the following notation. For each $i\in[n]$, we denote $\z_i:=y_i\x_i$ and $b_i:=y_ia_i\in\{\pm1\}$. We also let two vectors $\nub_{\pm}:=\begin{bmatrix} \mub_c \\ \pm\mub_{s} \end{bmatrix}\in\R^d$. 
Then, for all $i\in[n]$, we have 
\begin{align}
\z_i:=y_i\x_i=\nub_{b_i}+\q_i,\,\q_i\sim\Nn(0,I_d), i\in[n].
\end{align}
Recall also the notation
$$
\ellp_{i,t}:=\Delta_{g_i}\ell(\x_i^T\w^{t+1},g_i)=\Delta_{g_i}\omega_{g_i}e^{-\Delta_{g_i}\inp{\z_i}{\w}+\iota_{g_i}}
$$
%Motivated by this, it is convenient to split the training data into two subsets based on the value of $b=y\cdot a$, as follows:
%\begin{align}
%\Tc_1:=\Tc_{1,1}\cup\Tc_{-1,-1}\text{ and }\Tc_{-1}:=\Tc_{1,-1}\cup\Tc_{-1,1}.
%\end{align}
%Accordingly, let $n_{b}=|\Tc_b|,$ for $b\in\{\pm 1\}.$ Finally, denote
%\begin{align}
%R_+&:=\|\nub_{1}\|_2^2=\|\nub_{-1}\|_2^2={R_c^2+R_s^2}, \text{ and}\\
%R_-&:=\inp{\nub_{1}}{\nub_{-1}}=R_c^2-R_s^2.
%\end{align}
%Note that we might have $R_-<0$ if $R_s>R_c$, i.e., if the spurious features are more informative than the core ones. Also,  clearly $R_+\geq |R_-|$.




\subsection{Preliminary lemmas}

The following lemma shows that for the GMM of Section \ref{sec:GMM}, the per-group risk is a simple function of the correlation between the estimator and the corresponding mean vector. The proof is straightforward and is omitted for brevity.

\begin{lemma}[Worst-group error for GMM]
The per-group classification error of an estimator $\w$ can be bounded in terms of the correlation as follows:
\begin{align}
\Rwst=Q\big(\min_{b\in\{\pm 1\}}\inp{\nicefrac{\w}{\|\w\|_2}}{{\nub_{b}}}\big).
\end{align}
\end{lemma}

%\ct{Call $g_i:=y_ia_i$}

The next lemma is technical and it provides useful high-probability bounds on several quantities of interest under Assumption \ref{ass:dim}. 



\begin{lemma}[Good event $\Ec$]\label{lem:good}
There exists absolute constant $c_1\geq 1$ and $C_0:=C_0(c_1)>0$ such that the following statement holds for all problem parameters and success probability $1-\delta$ satisfying Assumptions \ref{ass-n} and \ref{ass-mu}. 
%Fix $\delta\in(0,1).$ There exists absolute constant $c_1\geq 1$, such that the following is true. For all large enough $C>0$ for which  Assumption \ref{ass:dim} holds,  
The following events hold simultaneously with probability $1-\delta$ for $b\in\{\pm1\}$:
% Further letting Assumption \ref{ass:dim} hold for $C>0$ and $\delta$, there exists constant $c_1>1$ such that with probability $1-\delta$ over the realization of the training set the data are linearly separable and the following events hold simultaneously for $b\in\{\pm1\}$,
\begin{align}
&\forall i\in\Tc_{b}\,:\,|\z_i^T\nub_b - R_+|\leq  R_+/2
\label{eq:zmu_same}
\\
&{\forall i\in\Tc_{-b}\,:\, |\z_i^T\nub_{b}- R_{-}| \leq c_1\sqrt{R_+}\sqrt{\log(n/\delta)}
\label{eq:zmu_same_sharp}}
\\
&\forall i\in[n]\,: \|\z_i\|_2^2 \leq c_1\dR
\label{eq:z_norm}
\\
&{\forall i\in[n]\,: \|\z_i\|_2 \geq \begin{cases}
(\sqrt{R_+}/c_1 -  \sqrt{d}) & R_+>c_1^2{d},\\
(\sqrt{d}/c_1 -  \sqrt{R_+}) & d>c_1^2{R_+}\\
\end{cases}
}
\label{eq:z_norm_lb}
\\
%\\
%&\red{\forall i\in[n]\,: |\|\z_i\|_2 - \sqrt{R_+}| \leq c_1\sqrt{d\log(n/\delta)} }
%\label{eq:z_norm}
%\\
%&\forall i\in\Tc_{b}, j\in\Tc_{-b}\,:|\z_i^T\z_j - R_-| \leq c_1\big(\sqrt{R_+}+\sqrt{d}\big) \sqrt{\log(n/\delta)}
%\label{eq:z_ortho}
%\\
&\forall \Tc_{b}\ni i\neq j\in\Tc_{\pm b}\,:|\z_i^T\z_j - {R_\pm}| \leq c_1\dRs\sqrt{\log(n/\delta)}
\label{eq:z_align}
\end{align}
When all the above holds, we say that good event $\Ec$ holds.
\end{lemma}


%\ct{Define $M:=\max\{d,R_+\}$.}
The proof of the lemma follows  
%by recognizing that for GMM data $\z_i=y_i\x_i=\mub_{a_i}+\q_i, \q_i\sim\Nn(0,I_d)$ and 
applying basic concentration inequalities, e.g. \cite{Verbook}. We omit the details due to space limits. 


\subsection{Key lemmas}
%Conditioned on the good event
%In the next section we present a lower bound on the correlation of the GD iterates conditioned on the good event $\Ec$ of Lemma \ref{lem:good}.


\begin{lemma}[Correlation lower bound]\label{lem:corrLB}Condition on the good event $\Ec$. 
For iteration $t$ and $b\in\{\pm1\}$, denote $\rho_{t,b}:=\inp{\w^t}{\nub_{b}}$ and $\Lpall:=\sum_{\tau=0}^t\Lpt:=\sum_{\tau=0}^t\sum_{i:b_i=b}\ellp_{i,\tau}$ for $b\in\{\pm1\}.$
Then, $\forall t>0$, the following bounds hold for $b\in{\pm1}$: 
 
%Refined inequalities: (useful???)
%\begin{align}\nn
%\rho_{t+1,b} &\geq \rho_{0,b}+\eta(R_+-c_1\sqrt{R_+}\sqrt{\log({n}/{\delta})})\Lpall\\
%&\qquad\quad+\eta(R_- -  c_1\sqrt{R_+}\sqrt{\log({n}/{\delta})}\Lpallneg
%\end{align}
\begin{align}\nn
\rho_{t+1,b} &\geq \rho_{0,b}+ {\eta\, R_+}\, \left( \frac{1}{2} \Lpall + 
\Big(\frac{R_-}{R_+} -  \frac{c_1}{C}\Big)\Lpallneg\right)
\end{align}
and
\begin{align}\nn
\|{\w^{t+1}}\|_2&\leq \|{\w^{0}}\|_2 + \eta \, c_1\,\dRs\,\big(\Lpallmaj+\Lpallmin\big).\nn
\end{align}

\end{lemma}
\begin{proof}
From GD iteration \eqref{eq:GD} together with Eqns. \eqref{eq:zmu_same},  \eqref{eq:zmu_diff}:
\begin{align*}
&\rho_{t+1,b}=\rho_{t,b}+\eta\sum_{i: b_i=b}\ellp_{i,\tau}\underbrace{\inp{\z_i}{\nub_b}}_{\geq R_+/2} \\
&\qquad\qquad + \eta \sum_{i: b_i=-b}\ellp_{i,\tau}\underbrace{\inp{\z_i}{\nub_{b}}}_{\geq R_--c_1\sqrt{R_+}\sqrt{\log(n/\delta)}} 
\\
&\qquad~ \geq \rho_{t,b} +\eta R_+\left(\frac{1}{2}\Lpt + \Big(\frac{R_-}{R_+}-\frac{c_1}{C}\Big)\Lptneg\right).
\end{align*}
In the last line above, we recalled the assumption $\sqrt{R_+}\geq C \sqrt{\log(n/\delta)}.$
The first inequality of the lemma follows from repeated application of the inequality in the above display for $\tau=0,\ldots,t+1.$ 

For the second inequality, apply again the GD iteration \eqref{eq:GD} together with triangle inequality and Eqn. \eqref{eq:z_norm} to find that
\begin{align*}
\|\w^{t+1}\|_2&=\|\w^{t}+\eta\sum_{i\in[n]}\ellp_{i,t}\z_i\|_2
\leq\|\w^{t}\|_2+\eta\sum_{i\in[n]}\ellp_{i,t}{\|\z_i\|_2}
\\&\leq\|\w^{t}\|_2+\eta c_1(\sqrt{R_+}+\sqrt{d}) \sum_{i\in[n]}\ellp_{i,t}
\end{align*}
In the second line above, we also used the fact that $\ellp_{i,t}\geq 0$. The desired follows by repeated application of this.
\end{proof}


\begin{lemma}[Gradients control]\label{lem:key}
In the good event $\Ec$, for all small step sizes and $\forall t\geq 0$, the following statement holds. If, the hyperparameters are all tuned as in the statement of Theorem \ref{thm:main}, then 
\begin{align}\label{eq:ellp_ratio}
\max_{i,j\in[n]}\Big\{\frac{\ellp_{i,t}}{\ellp_{j,t}}\Big\}\leq 4c_1^2 \frac{\Delta_{b_j}}{\Delta_{b_i}}.
\end{align}
\end{lemma}

%\ct{What if we relax (18) to avoid $d>R_+$?}



\subsection{Putting things together: Proof of Theorem \ref{thm:main}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:comparison}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Assume \eqref{eq:ellp_ratio} is true for all $t$. Then, there exists constant $c_0>0$ such that
\begin{align*}
c_0 \,\big(\Lptmaj+\Lptmin\big) \leq 
\frac{1}{2}\Lpt +\Big(\frac{R_-}{R_+}-\frac{c_1}{C}\Big)\Lptneg.
\end{align*}
%\red{provided that
%$$
%\frac{R_-}{R_+} \geq 0.
%$$
%}
\end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For simplicity denote $E:=\frac{R_-}{R_+}-\frac{c_1}{C}$.
 It suffices to show that
$
\big(1/2-c_0 \big)\Lpt \geq \big(c_0  - E\big)\Lptneg, 
$
or simpler:
\begin{align*}
\frac{\left(c_0-E \right)}{1/2-c_0} \leq \frac{n_{b}}{n_{-b}}\,\frac{\min_{i\in\Tc_{b}}\ellp_{t,i}}{\max_{i\in\Tc_{-b}}\ellp_{t,i}} \,.
\end{align*}
Recall now from \eqref{eq:ellp_ratio} and \eqref{eq:Delta} that $$\frac{\max_{i\in\Tc_{-b}}\ellp_{t,i}}{\min_{i\in\Tc_b}\ellp_{t,i}}\leq 4c_1^2\frac{\Delta_{b}}{\Delta_{-b}}\leq 16c_1^2 \frac{n_b}{n_{-b}}.$$
Hence, it suffices that
\begin{align*}
\frac{c_0-E }{1/2-c_0} \leq  \frac{1}{16c_1^2} \Leftarrow c_0 \leq \frac{1/2-16c_1^3/C+16c_1^2(R_-/R_+)}{1+16c_1^2}.
\end{align*}
Provided that $R_-/R_+\geq0$ and since $C$ can be set large enough (say relative to $c_1$), we can always choose positive $c_0$ satisfying the above.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Proof of Lemma \ref{lem:key}}

The conclusion of the lemma is obvious when $i=j$ since $c_1\geq 1$. For convenience let us fix pair of samples $(\x_1,a_1,y_1)$, $(\x_2,a_2,y_2)$ and call  
$
A_t := \frac{\ellp_{1,t}}{\ellp_{2,t}}. %\leq 2c_1^2 \frac{}{}
$
The same argument holds for any other pair of samples, thus the above restriction is without loss of generality.  
%
The proof is based on an induction argument. \ct{First, consider the base case $t=0$...} The base case for $t=0$ and $\w_0=0$, gives: $$A_0= \big({\omega_{b_1}\Delta_{b_1}e^{\iota_{b_1}}}\big)/\big({\omega_{b_2}\Delta_{b_2}e^{\iota_{b_2}}}\big). 
%{\exp({-\Delta_{b_1}\inp{\w_0}{\z_1}+\Delta_{b_2}\inp{\w_0}{\z_2}}}).
$$
Choosing $\omega_{b_1}=\omega_{b_2}=1$ and $\iota_{b_j}= \log(\Delta_{b_j}^{-2}), j=1,2$  yields $A_0\leq \Delta_{b_2}/\Delta_{b_1}\leq 4c_1^2\Delta_{b_2}/\Delta_{b_1},$ since $c_1>1.$


Next, assume that the statement of the lemma is true for iteration $t$. 
%
Our starting point to prove the statement for $t+1$ is the following recursion, obtained directly from the GD update rule:
\begin{align*}
&\frac{A_{t+1}}{A_t} =  \exp\left(-\eta\Delta_{b_1}\|\z_1\|^2\ellp_{1,t}+\eta\Delta_{b_2}\|\z_2\|^2\ellp_{2,t}\right) \\
&\cdot \exp\big(
-\eta\Delta_{b_1}\sum_{1\neq i\in[n]}\ellp_{i,t}\inp{\z_i}{\z_1}+
\eta\Delta_{b_2}\sum_{2\neq i\in[n]}\ellp_{i,t}\inp{\z_i}{\z_2}
\big)
\\
&\leq \exp\left(-\eta\Delta_{b_1}\|\z_1\|^2\ellp_{2,t}\,\Big(\frac{\ellp_{1,t}}{\ellp_{2,t}} - \frac{\|\z_2\|^2}{\|\z_1\|_2^2}\frac{\Delta_{b_2}}{\Delta_{b_1}}\Big)\right) \\
&\quad\cdot \exp\Big(\eta\Delta_{b_2}\ellp_{2,t}\big(\frac{\Delta_{b_1}}{\Delta_{b_2}}S_{1,+}+\frac{\Delta_{b_1}}{\Delta_{b_2}}S_{1,-}+S_{2,+}+S_{2,-}\big)\Big), \label{eq:recursion}
\end{align*}
where we set for  $j=1,2$, 
$
S_{j,\pm} = \sum_{i\neq j:b_i=\pm b_j}\frac{\ellp_{i,t}}{\ellp_{2,t}}|\inp{\z_i}{\z_j}|.
$
Now, note from applying Eqn. \eqref{eq:z_align} that 
$$
\max_{i\neq j:b_i=\pm b_j} |\inp{\z_i}{\z_j}| \leq U_{\pm},
$$
where, we set $U:=R_++c_1\dRs\sqrt{\log(n/\delta)}$ and we used that $R_+\geq R_-.$  Moreover, using the induction hypothesis for iteration $t$:
\begin{align}
\sum_{i\neq j:b_i=\pm b_j}\frac{\ellp_{i,t}}{\ellp_{2,t}} \leq  n_{\pm b_j}  \cdot \max_{i\in \Tc_{\pm b_j}}\frac{\ellp_{i,t}}{\ellp_{2,t}} \nn
&\leq n_{\pm b_j}  \cdot \frac{\Delta_{b_2}}{\Delta_{\pm b_j}}. \nn
\end{align}

Combining, the above three displays, we have shown that
\begin{align}
&\frac{\Delta_{b_1}}{\Delta_{b_2}}S_{1,+}+\frac{\Delta_{b_1}}{\Delta_{b_2}}S_{1,-}+S_{2,+}+S_{2,-} 
\\
\nn&\leq  U\big( n_{b_1} +  n_{-b_1} \frac{\Delta_{b_1}}{\Delta_{-b_1}} +  n_{b_2} +  n_{-b_2} \frac{\Delta_{b_2}}{\Delta_{-b_2}}\big) 
\\ 
 &\leq U\big(n_{b_1}+n_{b_2} + 4 n_{b_1} + 4 n_{b_2} \big) 
 \leq 5\,U\,n. \label{eq:2nd_bracket}
\end{align}
To obtain the penultimate inequality, we used the tuning of $\Delta$'s in \eqref{eq:Delta}. 

Now, using \eqref{eq:2nd_bracket} and the fact that $d/c_1\leq \|\z_1\|_2^2\leq c_1d$, we conclude with the following bound:
\begin{align}
&\log\frac{A_{t+1}}{A_{t}} \leq 
-\frac{\eta}{c_1}\Delta_{b_2}\ellp_{2,t}\, d\,\Big(
\frac{\Delta_{b_1}\ellp_{1,t}}{\Delta_{b_2}\ellp_{2,t}} - c_1^2-5c_1\,\frac{U\,n}{d}
\Big)\label{eq:log_1}
%\\
%&\leq
%\Delta_{b_1}\frac{d}{c_1}\ellp_{2,t}\big(\frac{\ellp_{1,t}}{\ellp_{2,t}} - \frac{1}{c_1^2}\frac{\Delta_{b_2}}{\Delta_{b_1}}\big) + 5\eta\Delta_{b_2}\ellp_{2,t}Un
\end{align}
At this point, we invoke Assumptions \ref{ass-d1} and \ref{ass-d2}. Specifically, choose $C_0=10(1+c_1)/c_1.$ Then, for all large enough $C>C_0$, it holds that $Un/d\leq (1+c_1)/C_0\leq c_1^2/10.$ Therefore, from \eqref{eq:log_1}:
\begin{align}
&\log\frac{A_{t+1}}{A_{t}} \leq 
-\frac{\eta}{c_1} \Delta_{b_2}\ellp_{2,t}\, d\,\Big(
\frac{\Delta_{b_1}\ellp_{1,t}}{\Delta_{b_2}\ellp_{2,t}} -\frac{3}{2}c_1^2
\Big)\label{eq:log_2}.
\end{align}
Finally, we distinguish two cases as follows. 

If $A_t\geq 2 c_1^2\Delta_{b_2}/\Delta_{b_1}$, then the parenthesis in the RHS of Eqn. \eqref{eq:log_2} is equal to $c_1^2/2>0$. Hence, in this case $A_{t+1}\leq A_t\leq 4c_1^2\Delta_{b_2}/\Delta_{b_1}$ as desired.

If the above does not hold, then $A_t< 2 c_1^2\Delta_{b_2}/\Delta_{b_1}$.  In this case \eqref{eq:log_2} can be further upper bounded as follows:
\begin{align*}
\log\frac{A_{t+1}}{A_{t}} \leq  \frac{3c_1}{2}\,{\eta}\, \Delta_{b_2}\,\ellp_{2,t}\, d \leq 6c_1\,\eta\,\frac{d}{n}\sum_{i\in[n]}\ell_{i,t} \leq 6c_1\,\eta\,{d}
\end{align*}
In the second inequality, we recalled that $\ellp_{2,t}=\Delta_{b_2}\ell_{2,t}$ and also used \eqref{eq:Delta}. The third inequality follows because the total loss is non-increasing at every $t$: $\sum_{i\in[n]}\ell_{i,t}\leq \sum_{i\in[n]}\ell_{i,0}=n$. \ct{Show!} Now, choosing small enough step-size $\eta\leq 1/(10c_1\,d)$, we find that $\log\frac{A_{t+1}}{A_{t}}\leq \log 2$, which implies $A_{t+1}\leq 2A_t\leq 4 c_1^2\Delta_{b_2}/\Delta_{b_1}$. 

In both cases, the desired inequality is proven.
%Next, using $d/c_1\leq \|\z_1\|_2^2\leq c_1d$ and $|\inp{\z_j}{\z_i}|\leq \|\mub_{a_j}\|_2^2+\sqrt{d\log(n/\delta)}, \forall i\neq j$, gives
%\begin{align}
%\nn&A_{t+1}\leq A_t  \cdot \exp\left(-\eta\frac{d}{c_1}\Delta_{b_1}\ellp_{2,t}\big(\frac{\ellp_{1,t}}{\ellp_{2,t}}-c_1^2\frac{\Delta_{b_2}}{\Delta_{b_1}}\big)\right) \\
%\nn&\cdot \exp\big(
%\eta\Delta_{b_1}(\|\mub_{a_1}\|_2^2+\sqrt{d\log(n/\delta)})\sum_{1\neq i\in[n]}\ellp_{i,t}\\
%&\eta\Delta_{b_2}(\|\mub_{a_2}\|_2^2+\sqrt{d\log(n/\delta)})\sum_{2\neq i\in[n]}\ellp_{i,t} \label{eq:rec}
%\big)
%\end{align}
%We will use the above to prove that 
%\begin{align}\label{eq:desired At}
%A_t={\ellp_{1,t}}/{\ellp_{2,t}}\leq 4c_1^2\big({\Delta_{b_2}}/{\Delta_{b_1}}\big).
%\end{align}
%
%\vp
%\noindent\underline{\emph{Case 1: $A_t\leq 2c_1^2\Delta_{b_2}/\Delta_{b_1}.$}}
%Continuing from \eqref{eq:rec} and recalling that $\ellp_{i,t}=\Delta_{y_i,a_i}\ell_{i,t}$, we find 
%\begin{align}
%&\frac{A_{t+1}}{A_t}\leq \exp\Big( 
%\eta \big(c_1 d \Delta_{b_2}^2 \ell_{2,t} \nn + (\Delta_{b_1}\vee\Delta_{b_2})^2\cdot \\
%&\qquad\cdot\big((\|\mub_1\|\vee\|\mub_{-1}\|)^2+\sqrt{d\log(n/\delta)} \big) \sum_{i\in[n]}\ell_{i,t} \big)
%\Big)\nn.
%\end{align}
%Further note that $\sum_{i\in[n]}\ell_{i,t}\leq \sum_{i\in[n]}\ell_{i,0}=n$ \ct{(to prove)}.
%By choosing sufficiently small step size $\eta$, we can guarantee that $\frac{A_{t+1}}{A_t}\leq \exp(1/2)\leq 2$. Thus, the desired \eqref{eq:desired At} follows.
%
%
%\vp
%\noindent\underline{\emph{Case 2: $A_t\geq 2c_1^2\Delta_{b_2}/\Delta_{b_1}.$}}
%Continuing from \eqref{eq:rec} and using our assumption
%\begin{align}
%&\frac{A_{t+1}}{A_t}\leq \exp\Big(- 
%\eta c_1 \Delta_{b_2} \ellp_{2,t}\big(R_--T_1/c_1-T_2/c_1\big)\Big)
%\end{align}
%where
%\begin{align*}
%&T_1 := (\|\mub_{a_1}\|_2^2+\sqrt{d\log(n/\delta)})\frac{\Delta_{b_1}}{\Delta_{b_2}}\sum_{1\neq i\in[n]}\frac{\ellp_{i,t}}{\ellp_{2,t}}\\
%&T_2 :=(\|\mub_{a_2}\|_2^2+\sqrt{d\log(n/\delta)})\sum_{2\neq i\in[n]}\frac{\ellp_{i,t}}{\ellp_{2,t}} 
%\end{align*}
%Using the induction hypothesis: 
%\begin{align*}
%&T_1 \leq 4c_1^2 (\|\mub_{a_1}\|_2^2+\sqrt{d\log(n/\delta)})\sum_{1\neq i\in[n]}\frac{\Delta_{b_1}}{\Delta_{y_i,a_i}}\\
%&T_2 \leq 4c_1^2(\|\mub_{a_2}\|_2^2+\sqrt{d\log(n/\delta)})\sum_{2\neq i\in[n]}\frac{\Delta_{b_2}}{\Delta_{y_i,a_i}}
%\end{align*}
%Note that for $j=1,2$
%\begin{align*}
%\sum_{1\neq i\in[n]}\frac{\Delta_{y_j,a_j}}{\Delta_{y_i,a_i}} &= \sum_{(y,a)\in(\pm1,\pm1)}\frac{\Delta_{y_j,a_j}}{\Delta_{y,a}}{n_{y,a}} 
%\\
%&\leq 2 \sum_{(y,a)\in(\pm1,\pm1)}{n_{y_j,a_j}} = 8 {n_{y_j,a_j}}.
%\end{align*}
%
%We need 
%\begin{align}
%d>C\max\{\|\mub_{a}\|_2^2(n_{1,a}+n_{-1,a}),n^2{\log(n/\delta)}\}.
%\end{align}





==> proofs2.tex <==
%%

%%--------------------------- NOTATION -------------------------------------
%\ct{If needed add a Table for notations. Too much :)}
This section includes the proof of Theorem \ref{thm:main}. Without further explicit reference, we assume $n$ training data generated as in Assumption \ref{ass:means}. For convenience, we introduce the following notation. For each $i\in[n]$, we denote $\z_i:=y_i\x_i$ and $b_i:=y_ia_i\in\{\pm1\}$. We also let two vectors $\nub_{\pm}:=\begin{bmatrix} \mub_c \\ \pm\mub_{s} \end{bmatrix}\in\R^d$. 
Then, for all $i\in[n]$, we have 
\begin{align} \label{eq:zmodel}
\z_i:=y_i\x_i=\nub_{b_i}+\q_i,\,\q_i\sim\Nn(0,I_d), i\in[n].
\end{align}
Recall also the notation
$$
\ellp_{i,t}:=\Delta_{g_i}\ell(\x_i^T\w^{t+1},g_i)=\Delta_{g_i}\omega_{g_i}e^{-\Delta_{g_i}\inp{\z_i}{\w}+\iota_{g_i}}
$$
In addition, throughout this sections, we use the following shorthand notations for iteration $t$ and $b\in\{\pm1\}$,
\begin{align*}
	\rho_{t,b}&:=\inp{\w^t}{\nub_{b}}\\
	\Lpt&:=\sum_{i:b_i=b}\ellp_{i,\tau}\\
	\Lpall&:=\sum_{\tau=0}^t\Lpt:=\sum_{\tau=0}^t\sum_{i:b_i=b}\ellp_{i,\tau}\\
	\Lpts&:=\sum_{i=1}^n\ellp_{i,\tau} = \Lpt + \Lptneg\\
	\Lpalls&:=\sum_{\tau=0}^t\Lpts:=\sum_{\tau=0}^t\sum_{i=1}^n\ellp_{i,\tau}\\
\end{align*} 
%Motivated by this, it is convenient to split the training data into two subsets based on the value of $b=y\cdot a$, as follows:
%\begin{align}
%\Tc_1:=\Tc_{1,1}\cup\Tc_{-1,-1}\text{ and }\Tc_{-1}:=\Tc_{1,-1}\cup\Tc_{-1,1}.
%\end{align}
%Accordingly, let $n_{b}=|\Tc_b|,$ for $b\in\{\pm 1\}.$ Finally, denote
%\begin{align}
%R_+&:=\|\nub_{1}\|_2^2=\|\nub_{-1}\|_2^2={R_c^2+R_s^2}, \text{ and}\\
%R_-&:=\inp{\nub_{1}}{\nub_{-1}}=R_c^2-R_s^2.
%\end{align}
%Note that we might have $R_-<0$ if $R_s>R_c$, i.e., if the spurious features are more informative than the core ones. Also,  clearly $R_+\geq |R_-|$.



\tina{Fix the order of the lemmas!}
\subsection{Preliminary lemmas}

%%--------------------------- WORST GROUP ERROR -------------------------------------

The following lemma shows that for the GMM of Section \ref{sec:GMM}, the per-group risk is a simple function of the correlation between the estimator and the corresponding mean vector.

\begin{lemma}[Worst-group error for GMM] \label{lem:wsterror}
	The per-group classification error of an estimator $\w$ can be bounded in terms of the correlation as follows:
	\begin{align}
	\Rwst=Q\big(\min_{b\in\{\pm 1\}}\inp{\nicefrac{\w}{\|\w\|_2}}{{\nub_{b}}}\big).
	\end{align}
\end{lemma}

%\ct{Call $g_i:=y_ia_i$}
\begin{proof}
	We start by the definition of $\Rwst$ from (\ref{eq:worst}) and the data model described in (\ref{eq:zmodel}),
	\begin{align*}
		\Rwst &= \max_{b \in \{\pm 1\}} P_{(\x,a,y) \sim \Pc} \Big(\inp{\nicefrac{\w}{\|\w\|_2}}{\z} < 0 \cond ay=b \Big)\\
		&= \max_{b \in \{\pm 1\}} P_{\q \sim \Nn(0,I_d)} \Big(\inp{\nicefrac{\w}{\|\w\|_2}}{\nub_{b}} < \inp{\nicefrac{\w}{\|\w\|_2}}{\q} \Big)\\
		&= \max_{b \in \{\pm 1\}} P_{\epsilon \sim \Nn(0,1)} \Big(\inp{\nicefrac{\w}{\|\w\|_2}}{\nub_{b}} < \epsilon \Big)\\
		&= \max_{b \in \{\pm 1\}} Q \Big(\inp{\nicefrac{\w}{\|\w\|_2}}{\nub_{b}}\Big)\\
		&= Q\big(\min_{b\in\{\pm 1\}}\inp{\nicefrac{\w}{\|\w\|_2}}{{\nub_{b}}}\big)
	\end{align*}
	\tina{fix notation: \ref{eq:worst} and maybe \ref{eq:zmodel}}
\end{proof}



%%--------------------------- CONCENTRATION INEQ & GOOD EVENT -----------------------------
The next lemma is technical and it provides useful high-probability bounds on several quantities of interest under Assumption \ref{ass:dim}. 




\begin{lemma}[Good event $\Ec$]\label{lem:good}
	There exists absolute constant $c_1\geq 1$ and $C_0:=C_0(c_1)>0$ such that the following statement holds for all problem parameters and success probability $1-\delta$ satisfying Assumptions \ref{ass-n} and \ref{ass-mu}. 
	%Fix $\delta\in(0,1).$ There exists absolute constant $c_1\geq 1$, such that the following is true. For all large enough $C>0$ for which  Assumption \ref{ass:dim} holds,  
	The following events hold simultaneously with probability $1-\delta$ for $b\in\{\pm1\}$:
	% Further letting Assumption \ref{ass:dim} hold for $C>0$ and $\delta$, there exists constant $c_1>1$ such that with probability $1-\delta$ over the realization of the training set the data are linearly separable and the following events hold simultaneously for $b\in\{\pm1\}$,
	\begin{align}
	&\forall i\in\Tc_{b}\,:\,|\z_i^T\nub_b - R_+|\leq  R_+/2
	\label{eq:zmu_same}
	\\
	&{\forall i\in\Tc_{-b}\,:\, |\z_i^T\nub_{b}- R_{-}| \leq c_1\sqrt{R_+}\sqrt{\log(n/\delta)}
		\label{eq:zmu_same_sharp}}
	\\
	&\forall i\in[n]\,: \|\z_i\|_2^2 \leq c_1 d
	\label{eq:z_norm}
	\\
	&\forall i\in[n]\,: \|\z_i\|_2^2 \geq d/c_1
	\label{eq:z_norm_lb}
	\\
	%\\
	%&\red{\forall i\in[n]\,: |\|\z_i\|_2 - \sqrt{R_+}| \leq c_1\sqrt{d\log(n/\delta)} }
	%\label{eq:z_norm}
	%\\
	%&\forall i\in\Tc_{b}, j\in\Tc_{-b}\,:|\z_i^T\z_j - R_-| \leq c_1\big(\sqrt{R_+}+\sqrt{d}\big) \sqrt{\log(n/\delta)}
	%\label{eq:z_ortho}
	%\\
	&\forall \Tc_{b}\ni i\neq j\in\Tc_{\pm b}\,:|\z_i^T\z_j - {R_\pm}| \leq c_1\sqrt{d}\sqrt{\log(n/\delta)}
	\label{eq:z_align}
	\end{align}
	When all the above holds, we say that good event $\Ec$ holds.
\end{lemma}
\begin{proof}
	\tina{...}
\end{proof}

%%--------------------------- DATA SEPARABILITY -------------------------------------
\begin{lemma}[Data separability and max-margin]\label{lem:maxmarg} \tina{check!}
	For any $\delta\in(0,1)$, there exists large enough constants $C_i>0$ such that with probability at least $1-\delta$ the training data are linearly separable, provided that $d\geq C_1\|\mub_c\|_2^2 n$, $\|\mub_c\|_2\geq C_2\sqrt{\log(n/\delta)}$ and $n\geq C_3$. Moreover, under the same conditions, with probability $1-\delta$ the maximum margin is lower bounded as follows for some constant $c>0$:
	\begin{align}
	\max_{\|\w\|=1}\min_{i\in[n]} \inp{\w}{\z_i} \geq c_2\sqrt{\frac{d}{n}}\,.
	\end{align}
\end{lemma}

\begin{proof}
	Recall the notation following notation for $i\in[n]$:
	$$
	\z_i:=\begin{bmatrix}
	\z_{i,c} \\
	\z_{i,s}
	\end{bmatrix} := y_i\begin{bmatrix}
	\x_{i,c} \\
	\x_{i,s}
	\end{bmatrix} = \begin{bmatrix}
	\mub_c + \q_{i,c}\\
	(y_ia_i)\,\mub_s + \q_{i,s}
	\end{bmatrix} 
	$$
	where $\q_{i,c},\q_{i,s}\sim\Nn(0,I_d)$  and independent of each other. We will prove that 
	$$
	\wt:= \sum_{i\in[n]}\begin{bmatrix}
	\z_{i,c} \\
	0
	\end{bmatrix}
	$$
	is a linear separator under the lemma's assumptions.
	Indeed, we have for any $j\in[n]$:
	\begin{align}
	\inp{\wt}{\z_j} = \|\z_{j,c}\|^2 + \inp{\z_{j,c}}{\sum_{j\neq i}\z_{i,c}}.
	\end{align}
	In the sequel, $c_1>1$ is a constant. First, with probability at least $1-\delta/2$ it holds simultaneously for all $j\in[n]$ that:
	\begin{subequations}\label{eq:event_sep}
		\begin{align}
		%\|\z_{j,c}\| &\geq \|\mub_c\| - c_1\sqrt{d \log(n/\delta)},\\
		&d/c_1 \leq \|\z_{j,c}\|^2 \leq c_1 d,\\
		&\inp{\z_{j,c}}{\mub_c}\leq \|\mub_c\|_2^2 + c_1\|\mub_c\|\sqrt{\log(n/\delta)}.
		\end{align}
	\end{subequations}
	Above, the first inequality holds because for large enough $C$, by assumption $d>C\|\mub\|_2^2$ and $\log(n/\delta)\geq C$.
	Second, since $\z_{i,c}, i\in[n]$ are i.i.d, we have that $\sum_{j\neq i}\z_{i,c}\sim\Nn((n-1)\mub_c,\sqrt{n}I_d)$ and is independent of $\z_{j,c}.$ Hence, conditioned on $\z_{j,c}$:
	$$
	\inp{\z_{j,c}}{\sum_{j\neq i}\z_{i,c}} \stackrel{(P)}{=}(n-1)\inp{\z_{j,c}}{\mub_c} + \| \z_{j,c}\|_2 \sqrt{n-1}\cdot G_j,\text{ with } G_j\sim\Nn(0,1).
	$$
	Thus, in the event \eqref{eq:event_sep}, with probability $1-\delta/2$, simultaneously for all $j\in[n]$:
	$$
	\inp{\z_{j,c}}{\sum_{j\neq i}\z_{i,c}}\leq n\|\mub_c\|_2^2 + c_1\|\mub_c\|n\sqrt{\log(n/\delta)}+c_1\sqrt{d n}\sqrt{\log(n/\delta)}.
	$$
	Putting things together, with probability at least $1-\delta$, simultaneously for all $j\in[n]$, it holds that
	\begin{align*}
	&\frac{1}{n}\inp{\wt}{\z_j} \geq \frac{d}{c_1 n} 
	\\ &\quad-\Big(\|\mub_c\|^2 + c_1\|\mub_c\|\sqrt{\log(n/\delta)}+c_1\sqrt{\frac{d{\log(n/\delta)}}{n}}\Big)
	\end{align*}
	By invoking $\sqrt{\log(n/\delta)}\leq \|\mub_c\|/C_2$ for some constant $C_2>0$ and picking large enough $C_1$ such that $d/n\geq C_1 \|\mub_c\|^2$, this shows that for some $c'>1$:
	\begin{align}\label{eq:inp_bound_sep}
	\min_{i\in[n]} \inp{\wt}{\z_i} \geq d/c' >0.
	\end{align}
	Therefore, the $\wt$ is a linear separator. 
	
	Next, we upper bound the norm of $\wt$. With probability $1-\delta$:
	\begin{align}
	\|\wt\|_2 = \| n\mub_c + \sum_{i\in[n]}\q_{i,c}\| \leq n\|\mub_c\| + c_1\sqrt{n}\sqrt{d}
	\end{align}
	where the upper bound follows by triangle inequality and using that $\sum_{i\in[n]}\q_{i,c}\sim\Nn(0,\sqrt{n} I_d)$ to invoke Fact \ref{fact:g_norm}. Under the conditions of the lemma, $\|\mub_c\|\sqrt{n}\leq \sqrt{d}/\sqrt{C_1}$ . Hence,  for some $c''\geq 1$:
	\begin{align}\label{eq:norm_bound_sep}
	\|\wt\|_2  \leq c'' \sqrt{n}\sqrt{d}.
	\end{align}
	
	Putting together \eqref{eq:inp_bound_sep} and \eqref{eq:norm_bound_sep}, we conclude with the second statement of the lemma, i.e.
	$$
	\max_{\|\w\|=1}\min_{i\in[n]} \inp{\w}{\z_i}  \geq \frac{\min_{i\in[n]}\inp{\wt}{\z_j}}{\|\wt\|_2} \geq c_2 \sqrt{\frac{d}{n}}\,.
	$$
	
\end{proof}

\begin{lemma} \label{lem:GDprop}
	\tina{for GD step, norm w gets to infty and loss is decreasing}	
\end{lemma}

%%--------------------------- UPPER BOUND ON ||W|| -------------------------------------

%%--------------------------- LOWER BOUND ON CORRELATION -------------------------------------


%%--------------------------- LOWER BOUND ON ||W|| -------------------------------------

%%--------------------------- UPPER BOUND ON CORRELATION -------------------------------------

\subsection{Key lemmas}
%Conditioned on the good event
%In the next section we present a lower bound on the correlation of the GD iterates conditioned on the good event $\Ec$ of Lemma \ref{lem:good}.


\begin{lemma}[Correlation bounds]\label{lem:corrLB}
	Under Assumption \ref{ass:dim} and conditioned on the good event $\Ec$, for all iteration $t > 0$ and $b\in\{\pm1\}$, the following bounds hold:
	
%	Condition on the good event $\Ec$. 
%	For iteration $t$ and $b\in\{\pm1\}$, denote $\rho_{t,b}:=\inp{\w^t}{\nub_{b}}$ and $\Lpall:=\sum_{\tau=0}^t\Lpt:=\sum_{\tau=0}^t\sum_{i:b_i=b}\ellp_{i,\tau}$ for $b\in\{\pm1\}.$
%	Then, $\forall t>0$, the following bounds hold for $b\in{\pm1}$: 
%	
	%Refined inequalities: (useful???)
	%\begin{align}\nn
	%\rho_{t+1,b} &\geq \rho_{0,b}+\eta(R_+-c_1\sqrt{R_+}\sqrt{\log({n}/{\delta})})\Lpall\\
	%&\qquad\quad+\eta(R_- -  c_1\sqrt{R_+}\sqrt{\log({n}/{\delta})}\Lpallneg
	%\end{align}
	\begin{align}
	\rho_{t+1,b} &\geq \rho_{0,b}+ {\eta\, R_+}\, \left( \frac{1}{2} \Lpall + 
	\Big(\frac{R_-}{R_+} -  \frac{c_1}{C}\Big)\Lpallneg\right) \label{eq:corrLB}
	\end{align}
	and
	\begin{align}
	\|{\w^{t+1}}\|_2&\leq \|{\w^{0}}\|_2 + \eta \, c_1\,\sqrt{d}\,\Lpalls\,. \label{eq:normUB}
	\end{align}
	
\end{lemma}
\begin{proof}
	From GD iteration \eqref{eq:GD} together with Eqns. \eqref{eq:zmu_same},  \eqref{eq:zmu_diff}:
	
	\begin{align*}
		\rho_{t+1,b} &= \rho_{t,b}+\eta\sum_{i: b_i=b}\ellp_{i,\tau}\inp{\z_i}{\nub_b} + 
		\eta \sum_{i: b_i=-b}\ellp_{i,\tau}\inp{\z_i}{\nub_{b}} \\
		&\geq \rho_{t,b} +\eta\sum_{i: b_i=b}\ellp_{i,\tau} \frac{R_+}{2} \\ 
		& \qquad \quad + \eta \sum_{i: b_i=-b}\ellp_{i,\tau} \big(R_--c_1\sqrt{R_+}\sqrt{\log(n/\delta)} \big)\\
		&\geq \rho_{t,b} +\eta R_+\left(\frac{1}{2}\Lpt + \Big(\frac{R_-}{R_+}-\frac{c_1}{C}\Big)\Lptneg\right).
	\end{align*}
	
%	\begin{align*}
%	&\rho_{t+1,b}=\rho_{t,b}+\eta\sum_{i: b_i=b}\ellp_{i,\tau}\underbrace{\inp{\z_i}{\nub_b}}_{\geq R_+/2} \\
%	&\qquad\qquad + \eta \sum_{i: b_i=-b}\ellp_{i,\tau}\underbrace{\inp{\z_i}{\nub_{b}}}_{\geq R_--c_1\sqrt{R_+}\sqrt{\log(n/\delta)}} 
%	\\
%	&\qquad~ \geq \rho_{t,b} +\eta R_+\left(\frac{1}{2}\Lpt + \Big(\frac{R_-}{R_+}-\frac{c_1}{C}\Big)\Lptneg\right).
%	\end{align*}
	In the last line above, we recalled the assumption $\sqrt{R_+}\geq C \sqrt{\log(n/\delta)}.$
	The first inequality of the lemma follows from repeated application of the inequality in the above display for $\tau=0,\ldots,t+1.$ 
	
	For the second inequality, apply again the GD iteration \eqref{eq:GD} together with triangle inequality and Eqn. \eqref{eq:z_norm} to find that
	\begin{align*}
	\|\w^{t+1}\|_2&=\|\w^{t}+\eta\sum_{i\in[n]}\ellp_{i,t}\z_i\|_2
	\leq\|\w^{t}\|_2+\eta\sum_{i\in[n]}\ellp_{i,t}{\|\z_i\|_2}
	\\&\leq\|\w^{t}\|_2+\eta c_1 \,\sqrt{d} \sum_{i\in[n]}\ellp_{i,t}
	\end{align*}
	In the second line above, we also used the fact that $\ellp_{i,t}\geq 0$. The desired follows by repeated application of this.
\end{proof}



\begin{lemma}
	Assuming we have a realization of a good event $\Ec$, there exist $t_0>0$ and $c', c''>0$ such that for all iteration $t>t_0$ and $b \in \{\pm 1\}$,
	\begin{align}
		\rho_{t+1,b} &\leq \rho_{t_0,b} +\eta R_+\left(\frac{3}{2}L^\prime_{t_0:t,b} + \Big(\frac{R_-}{R_+}+\frac{c_1}{C}\Big)L^\prime_{t_0:t,-b}\right) \label{eq:corrtheorem2} \\	
		\|\w^{t+1}\|_2 &\geq \|\w^{t_0}\|_2 + \frac{\eta c_2}{4} \, \sqrt{\frac{d}{n}} L^\prime_{t_0:t} \label{eq:normtheorem2}
	\end{align}
%	\begin{align}
%	\rho_{t+1,b} &\leq \rho_{t_0,b} + \eta c' R_+ \Big(\frac{n_b}{n_{-b}} + \frac{R_-}{R_+} + c_1\sqrt{\frac{\log(n/\delta)}{R_+}}\Big) L^\prime_t \label{eq:corrtheorem2}\\
%	\|\w^{t}\|_2 &\geq \|\w^{t_0}\|_2+\eta c''\sqrt{\frac{d}{n}}L^\prime_t \label{eq:normtheorem2}
%	\end{align}
\end{lemma}

\begin{proof}
	By the application of gradient descent steps and equations \eqref{eq:zmu_same} and \eqref{eq:zmu_same_sharp},
	\begin{align*}
		\rho_{t+1,b} &= \rho_{t,b}+\eta\sum_{i: b_i=b}\ellp_{i,\tau}\inp{\z_i}{\nub_b} + 
		\eta \sum_{i: b_i=-b}\ellp_{i,\tau}\inp{\z_i}{\nub_{b}} \\
		&\leq \rho_{t,b}+\eta\sum_{i: b_i=b}\ellp_{i,\tau} \frac{3R_+}{2} \\ 
		& \qquad \quad + \eta \sum_{i: b_i=-b}\ellp_{i,\tau} \big(R_-+c_1\sqrt{R_+}\sqrt{\log(n/\delta)} \big)\\
		& \leq \rho_{t,b} +\eta R_+\left(\frac{3}{2}\Lpt + \Big(\frac{R_-}{R_+}+\frac{c_1}{C}\Big)\Lptneg\right).
	\end{align*}
%	\begin{align*}
%	\rho_{t+1,b} &- \rho_{t,b} \leq \eta \Big[\sum_{i\in\Tc_{b}} \ellp_{i,t} \inp{\z_i}{\nub_b}
%	+ \sum_{i\in\Tc_{-b}} \ellp_{i,t} \inp{\z_i}{\nub_b}
%	\Big]\\
%	&\leq c_2\eta\Big[\frac{3R_+}{2} \frac{n_b}{n} + (R_-+c_1\sqrt{R_+ \log(n/\delta)}) \frac{n_{-b}}{n} \Big] L^\prime _t\\
%	&\leq \eta c^\prime R_+ \Big[\frac{n_b}{n_{-b}} + \frac{R_-}{R_+} + c_1\sqrt{\frac{\log(n/\delta)}{R_+}} \Big] L^\prime _t
%	\end{align*}
	where in the second line we use Lemma \ref{lem:ratio2}. By repeating this inequality, equation \eqref{eq:corrtheorem2} is proven.
	
	For the second statement, from the gradient descent iteration:
	\begin{align}
	\|\w^{t+1}\|_2^2 &= \|\w^{t} + \eta\sum_{i=1}^n \ellp_{i,t} \z_i\|_2^2 \nonumber\\
	&\geq \|\w^{t}\|_2^2  + 2\eta\sum_{i=1}^n \ellp_{i,t} \inp{\z_i}{\w^t}
	\end{align}
	
	Based on Lemma \ref{lem:maxmarg}, the data is linearly separable, and based on \ref{lem:GDprop} \tina{complete!}. Thus, there exists $t_1 > 0$ such that for all $t>t_1$,
	
	\begin{align}
	\inp{\z_i}{\frac{\w^t}{\|\w^t\|_2}} \geq \frac{c_2}{2} \sqrt{\frac{d}{n}} \label{eq:GDmargin}
	\end{align}
	
	Combining equations \eqref{eq:norm} and \eqref{eq:lbcorr},
	\begin{align*}
	\|\w^{t+1}\|^2_2 &\geq \|\w^{t}\|^2_2 \bigg(1 + \eta c_2 \, \sqrt{\frac{d}{n}} \frac{L^\prime_t}{\|\w^t\|_2}\bigg)
	\end{align*}
	
	\tina{norm gets to infty} Hence, there exists $t_2>0$ such that for all $t>0$,
	\begin{align}\label{eq:GDnorm}
		\|\w^t\|_2 \geq \eta c_2 \, \sqrt{\frac{d}{n}}\frac{L^\prime_0}{8} \geq \eta c_2 \, \sqrt{\frac{d}{n}}\frac{L^\prime_t}{8}
	\end{align}
	Now, setting $t_0 = \max\{t_1,t_2\}$ to satisfy both \eqref{eq:GDmargin} and \eqref{eq:GDnorm}, we have,
	\begin{align*}
		\|\w^{t+1}\|^2_2 &\geq \Big(\|\w^{t}\|_2 + \frac{\eta c_2}{4} \, \sqrt{\frac{d}{n}} L^\prime_t\Big)^2
	\end{align*}
%	[??] further show that the loss function at GD steps will be decreasing during training, and as $t$ increases, $\norm{\w^t}_2$ gets to $\infty$. Therefore, as $\norm{\w^0}_2 = 0$, $L^\prime_t \leq \sum_{i=0}^n \omega_{g_i}e^{\iota_{g_i}}$, and after a point in the training, 
%	\begin{align}\label{eq:GDnorm}
%	\norm{\w^t}_2 \geq \frac{\eta c''' \sqrt{\frac{d}{n}}	\sum_{i=0}^n \omega_{g_i}e^{\iota_{g_i}}}{8}
%	\end{align}
	
%	Assuming that $t_0$ is large enough to satisfy both \eqref{eq:GDmargin} and \eqref{eq:GDnorm}, for $t>t_0$ we have, 
%	\begin{align*}
%	\|\w^{t+1}\|_2 &\geq \|\w^{t}\|_2 + \eta c''\sqrt{\frac{d}{n}} \sum_{i=1}^n L^\prime_t
%	\end{align*}
	Finally, \eqref{eq:normtheorem2} follows by repeatedly applying this inequality.\\
	
\end{proof}

%%--------------------------- LOSS RATIO -------------------------------------
\begin{lemma}[Gradients control]\label{lem:key}
	In the good event $\Ec$, for all small step sizes and $\forall t\geq 0$, the following statement holds. If, the hyperparameters are all tuned as in the statement of Theorem \ref{thm:main}, then 
	\begin{align}\label{eq:ellp_ratio}
	\max_{i,j\in[n]}\Big\{\frac{\ellp_{i,t}}{\ellp_{j,t}}\Big\}\leq 4c_1^2 \frac{\Delta_{b_j}}{\Delta_{b_i}}.
	\end{align}
\end{lemma}

\begin{proof}
	The conclusion of the lemma is obvious when $i=j$ since $c_1\geq 1$. For convenience let us fix pair of samples $(\x_1,a_1,y_1)$, $(\x_2,a_2,y_2)$ and call  
	$
	A_t := \frac{\ellp_{1,t}}{\ellp_{2,t}}. %\leq 2c_1^2 \frac{}{}
	$
	The same argument holds for any other pair of samples, thus the above restriction is without loss of generality.  
	%
	The proof is based on an induction argument. The base case for $t=0$ and $\w_0=0$, gives: $$A_0= \big({\omega_{b_1}\Delta_{b_1}e^{\iota_{b_1}}}\big)/\big({\omega_{b_2}\Delta_{b_2}e^{\iota_{b_2}}}\big). 
	%{\exp({-\Delta_{b_1}\inp{\w_0}{\z_1}+\Delta_{b_2}\inp{\w_0}{\z_2}}}).
	$$
	Choosing $\omega_{b_1}=\omega_{b_2}=1$ and $\iota_{b_j}= \log(\Delta_{b_j}^{-2}), j=1,2$  yields $A_0\leq \Delta_{b_2}/\Delta_{b_1}\leq 4c_1^2\Delta_{b_2}/\Delta_{b_1},$ since $c_1>1.$
	
	
	Next, assume that the statement of the lemma is true for iteration $t$. 
	%
	Our starting point to prove the statement for $t+1$ is the following recursion, obtained directly from the GD update rule:
	\begin{align*}
	&\log \frac{A_{t+1}}{A_t} =  -\eta\Delta_{b_1}\|\z_1\|^2\ellp_{1,t}+\eta\Delta_{b_2}\|\z_2\|^2\ellp_{2,t} \\
	& -\eta\Delta_{b_1}\sum_{1\neq i\in[n]}\ellp_{i,t}\inp{\z_i}{\z_1}+
	\eta\Delta_{b_2}\sum_{2\neq i\in[n]}\ellp_{i,t}\inp{\z_i}{\z_2}
	\\
	&\leq -\eta\Delta_{b_2}\ellp_{2,t} \|\z_1\|^2\,\Big(\frac{\ellp_{1,t}}{\ellp_{2,t}} \frac{\Delta_{b_1}}{\Delta_{b_2}} - \frac{\|\z_2\|^2}{\|\z_1\|_2^2}\Big) 
	\\& + \eta\Delta_{b_2}\ellp_{2,t} \big(\frac{\Delta_{b_1}}{\Delta_{b_2}}S_{1,+}+\frac{\Delta_{b_1}}{\Delta_{b_2}}S_{1,-}+S_{2,+}+S_{2,-}\big), \label{eq:recursion}
	\end{align*}
	where we set for  $j=1,2$, 
	$
	S_{j,\pm} = \sum_{i\neq j:b_i=\pm b_j}\frac{\ellp_{i,t}}{\ellp_{2,t}}|\inp{\z_i}{\z_j}|.
	$
	Now, note from applying Eqn. \eqref{eq:z_align} that 
	$$
	\max_{i\neq j:b_i=\pm b_j} |\inp{\z_i}{\z_j}| \leq U,
	$$
	where, we set $U:=R_++c_1\sqrt{d}\sqrt{\log(n/\delta)}$ and we used that $R_+\geq R_-.$  Moreover, using the induction hypothesis for iteration $t$:
	\begin{align}
	\sum_{i\neq j:b_i=\pm b_j}\frac{\ellp_{i,t}}{\ellp_{2,t}} \leq  n_{\pm b_j}  \cdot \max_{i\in \Tc_{\pm b_j}}\frac{\ellp_{i,t}}{\ellp_{2,t}} \nn
	&\leq n_{\pm b_j}  \cdot \frac{\Delta_{b_2}}{\Delta_{\pm b_j}}. \nn
	\end{align}
	
	Combining, the above three displays, we have shown that
	\begin{align}
	&\frac{\Delta_{b_1}}{\Delta_{b_2}}S_{1,+}+\frac{\Delta_{b_1}}{\Delta_{b_2}}S_{1,-}+S_{2,+}+S_{2,-} 
	\\
	\nn&\leq  U\big( n_{b_1} +  n_{-b_1} \frac{\Delta_{b_1}}{\Delta_{-b_1}} +  n_{b_2} +  n_{-b_2} \frac{\Delta_{b_2}}{\Delta_{-b_2}}\big) 
	\\ 
	&\leq U\big(n_{b_1}+n_{b_2} + 4 n_{b_1} + 4 n_{b_2} \big) 
	\leq \red{10}\,U\,n. \label{eq:2nd_bracket}
	\end{align}
	To obtain the penultimate inequality, we used the tuning of $\Delta$'s in \eqref{eq:Delta}. 
	
	Now, using \eqref{eq:2nd_bracket} and the fact that $d/c_1\leq \|\z_1\|_2^2\leq c_1d$, we conclude with the following bound:
	\begin{align}
	&\log\frac{A_{t+1}}{A_{t}} \leq 
	-\frac{\eta}{c_1}\Delta_{b_2}\ellp_{2,t}\, d\,\Big(
	\frac{\Delta_{b_1}\ellp_{1,t}}{\Delta_{b_2}\ellp_{2,t}} - c_1^2-\red{10}c_1\,\frac{U\,n}{d}
	\Big)\label{eq:log_1}
	%\\
	%&\leq
	%\Delta_{b_1}\frac{d}{c_1}\ellp_{2,t}\big(\frac{\ellp_{1,t}}{\ellp_{2,t}} - \frac{1}{c_1^2}\frac{\Delta_{b_2}}{\Delta_{b_1}}\big) + 5\eta\Delta_{b_2}\ellp_{2,t}Un
	\end{align}
	At this point, we invoke Assumptions \ref{ass-d1} and \ref{ass-d2}. Specifically, choose $C_0=\red{10}(1+c_1)/c_1.$ Then, for all large enough $C>C_0$, it holds that $Un/d\leq (1+c_1)/C_0\leq c_1^2/\red{10}.$ Therefore, from \eqref{eq:log_1}:
	\begin{align}
	&\log\frac{A_{t+1}}{A_{t}} \leq 
	-\frac{\eta}{c_1} \Delta_{b_2}\ellp_{2,t}\, d\,\Big(
	\frac{\Delta_{b_1}\ellp_{1,t}}{\Delta_{b_2}\ellp_{2,t}} -\red{2}c_1^2
	\Big)\label{eq:log_2}.
	\end{align}
	Finally, we distinguish two cases as follows. 
	
	If $A_t\geq 2 c_1^2\Delta_{b_2}/\Delta_{b_1}$, then the parenthesis in the RHS of Eqn. \eqref{eq:log_2} is positive. Hence, in this case $A_{t+1}\leq A_t\leq 4c_1^2\Delta_{b_2}/\Delta_{b_1}$ as desired.
	
	If the above does not hold, then $A_t< 2 c_1^2\Delta_{b_2}/\Delta_{b_1}$.  In this case \eqref{eq:log_2} can be further upper bounded as follows:
	\begin{align*}
	&\log\frac{A_{t+1}}{A_{t}} \leq  \frac{3c_1}{2}\,{\eta}\, \Delta_{b_2}\,\ellp_{2,t}\, d \leq 6c_1\,\eta\,\frac{d}{n}\sum_{i\in[n]}\ell_{i,t} \leq 6c_1\,\eta\,{d}\\
	&\red{\log\frac{A_{t+1}}{A_{t}} \leq  \frac{2c_1}{1}\,{\eta}\, \Delta_{b_2}\,\ellp_{2,t}\, d \leq 8c_1\,\eta\,d\sum_{i\in[n]}\ell_{i,t} \leq 8c_1\,\eta\,dn}
	\end{align*}
	In the second inequality, we recalled that $\ellp_{2,t}=\Delta_{b_2}\ell_{2,t}$ and also used \eqref{eq:Delta}. The third inequality follows because the total loss is non-increasing at every $t$: $\sum_{i\in[n]}\ell_{i,t}\leq \sum_{i\in[n]}\ell_{i,0}=n$. \ct{Show!} Now, choosing small enough step-size $\red{\eta\leq 1/(10c_1\,d)}$, we find that $\log\frac{A_{t+1}}{A_{t}}\leq \log 2$, which implies $A_{t+1}\leq 2A_t\leq 4 c_1^2\Delta_{b_2}/\Delta_{b_1}$. 
	
	In both cases, the desired inequality is proven.
	%Next, using $d/c_1\leq \|\z_1\|_2^2\leq c_1d$ and $|\inp{\z_j}{\z_i}|\leq \|\mub_{a_j}\|_2^2+\sqrt{d\log(n/\delta)}, \forall i\neq j$, gives
	%\begin{align}
	%\nn&A_{t+1}\leq A_t  \cdot \exp\left(-\eta\frac{d}{c_1}\Delta_{b_1}\ellp_{2,t}\big(\frac{\ellp_{1,t}}{\ellp_{2,t}}-c_1^2\frac{\Delta_{b_2}}{\Delta_{b_1}}\big)\right) \\
	%\nn&\cdot \exp\big(
	%\eta\Delta_{b_1}(\|\mub_{a_1}\|_2^2+\sqrt{d\log(n/\delta)})\sum_{1\neq i\in[n]}\ellp_{i,t}\\
	%&\eta\Delta_{b_2}(\|\mub_{a_2}\|_2^2+\sqrt{d\log(n/\delta)})\sum_{2\neq i\in[n]}\ellp_{i,t} \label{eq:rec}
	%\big)
	%\end{align}
	%We will use the above to prove that 
	%\begin{align}\label{eq:desired At}
	%A_t={\ellp_{1,t}}/{\ellp_{2,t}}\leq 4c_1^2\big({\Delta_{b_2}}/{\Delta_{b_1}}\big).
	%\end{align}
	%
	%\vp
	%\noindent\underline{\emph{Case 1: $A_t\leq 2c_1^2\Delta_{b_2}/\Delta_{b_1}.$}}
	%Continuing from \eqref{eq:rec} and recalling that $\ellp_{i,t}=\Delta_{y_i,a_i}\ell_{i,t}$, we find 
	%\begin{align}
	%&\frac{A_{t+1}}{A_t}\leq \exp\Big( 
	%\eta \big(c_1 d \Delta_{b_2}^2 \ell_{2,t} \nn + (\Delta_{b_1}\vee\Delta_{b_2})^2\cdot \\
	%&\qquad\cdot\big((\|\mub_1\|\vee\|\mub_{-1}\|)^2+\sqrt{d\log(n/\delta)} \big) \sum_{i\in[n]}\ell_{i,t} \big)
	%\Big)\nn.
	%\end{align}
	%Further note that $\sum_{i\in[n]}\ell_{i,t}\leq \sum_{i\in[n]}\ell_{i,0}=n$ \ct{(to prove)}.
	%By choosing sufficiently small step size $\eta$, we can guarantee that $\frac{A_{t+1}}{A_t}\leq \exp(1/2)\leq 2$. Thus, the desired \eqref{eq:desired At} follows.
	%
	%
	%\vp
	%\noindent\underline{\emph{Case 2: $A_t\geq 2c_1^2\Delta_{b_2}/\Delta_{b_1}.$}}
	%Continuing from \eqref{eq:rec} and using our assumption
	%\begin{align}
	%&\frac{A_{t+1}}{A_t}\leq \exp\Big(- 
	%\eta c_1 \Delta_{b_2} \ellp_{2,t}\big(R_--T_1/c_1-T_2/c_1\big)\Big)
	%\end{align}
	%where
	%\begin{align*}
	%&T_1 := (\|\mub_{a_1}\|_2^2+\sqrt{d\log(n/\delta)})\frac{\Delta_{b_1}}{\Delta_{b_2}}\sum_{1\neq i\in[n]}\frac{\ellp_{i,t}}{\ellp_{2,t}}\\
	%&T_2 :=(\|\mub_{a_2}\|_2^2+\sqrt{d\log(n/\delta)})\sum_{2\neq i\in[n]}\frac{\ellp_{i,t}}{\ellp_{2,t}} 
	%\end{align*}
	%Using the induction hypothesis: 
	%\begin{align*}
	%&T_1 \leq 4c_1^2 (\|\mub_{a_1}\|_2^2+\sqrt{d\log(n/\delta)})\sum_{1\neq i\in[n]}\frac{\Delta_{b_1}}{\Delta_{y_i,a_i}}\\
	%&T_2 \leq 4c_1^2(\|\mub_{a_2}\|_2^2+\sqrt{d\log(n/\delta)})\sum_{2\neq i\in[n]}\frac{\Delta_{b_2}}{\Delta_{y_i,a_i}}
	%\end{align*}
	%Note that for $j=1,2$
	%\begin{align*}
	%\sum_{1\neq i\in[n]}\frac{\Delta_{y_j,a_j}}{\Delta_{y_i,a_i}} &= \sum_{(y,a)\in(\pm1,\pm1)}\frac{\Delta_{y_j,a_j}}{\Delta_{y,a}}{n_{y,a}} 
	%\\
	%&\leq 2 \sum_{(y,a)\in(\pm1,\pm1)}{n_{y_j,a_j}} = 8 {n_{y_j,a_j}}.
	%\end{align*}
	%
	%We need 
	%\begin{align}
	%d>C\max\{\|\mub_{a}\|_2^2(n_{1,a}+n_{-1,a}),n^2{\log(n/\delta)}\}.
	%\end{align}
	
\end{proof}


\begin{lemma}\label{lem:ratio2}[\red{Gradient Control LA Loss}]
	When a good event $\Ec$ holds, with sufficiently small step size, the following inequality is satisfied for all GD steps of LA-loss,
	\begin{align}
	\max_{i,j\in[n]}\Big\{\frac{\ellp_{i,t}}{\ellp_{j,t}}\Big\}\leq c_3
	\end{align} 
	where 
	\begin{align}
	c_3 = \max \{4c_1^2, \frac{\omega_+ e^{\iota_+}}{\omega_- e^{\iota_-}}, \frac{\omega_- e^{\iota_-}}{\omega_+ e^{\iota_+}}\}	\label{eq:lossratio_cond}
	\end{align}
\end{lemma}
Note again that LA-loss is equivalent to VS-loss when $\Delta_\pm=1$. Following the steps in the proof of Lemma \ref{lem:key}, we can prove this statement similarly.	\eqref{eq:lossratio_cond} is to make sure the base case of the induction is satisfied.
\tina{Gradient control bound has a subtle differnece because it is proven for any choice of iota and omega. The only difference in the proof is for the base case I guess. Can we merge them into one lemma or is it better to have two separate lemmas for it...?}


\subsection{Putting things together: Proof of Theorem \ref{thm:main}}
%%------------------------------ BOUNDING BY LOSS SUMMATION	---------------------------
\begin{lemma}\label{lem:comparison}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	Assume \eqref{eq:ellp_ratio} is true for all $t$. Then, there exists constant $c_0>0$ such that
	\begin{align*}
	c_0 \,\Lpts \leq 
	\frac{1}{2}\Lpt +\Big(\frac{R_-}{R_+}-\frac{c_1}{C}\Big)\Lptneg.
	\end{align*}
	%\red{provided that
	%$$
	%\frac{R_-}{R_+} \geq 0.
	%$$
	%}
\end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	For simplicity denote $E:=\frac{R_-}{R_+}-\frac{c_1}{C}$.
	It suffices to show that
	$
	\big(1/2-c_0 \big)\Lpt \geq \big(c_0  - E\big)\Lptneg, 
	$
	or simpler (\red{assuming $1/2-c_0>0$}):
	\begin{align*}
	&\frac{c_0-E}{1/2-c_0} \leq \frac{n_{b}}{n_{-b}}\,\frac{\min_{i\in\Tc_{b}}\ellp_{t,i}}{\max_{i\in\Tc_{-b}}\ellp_{t,i}} \,.
	\\&\red{\frac{\left(c_0-E \right)}{1/2-c_0} \leq \frac{\Lpt}{\Lptneg} \leq \frac{n_{b}}{n_{-b}}\,\frac{\max_{i\in\Tc_{b}}\ellp_{t,i}}{\min_{i\in\Tc_{-b}}\ellp_{t,i}} \,.}
	\end{align*}
	Recall now from \eqref{eq:ellp_ratio} and \eqref{eq:Delta} that
	\begin{align*}
		&\frac{\max_{i\in\Tc_{-b}}\ellp_{t,i}}{\min_{i\in\Tc_b}\ellp_{t,i}}\leq 4c_1^2\frac{\Delta_{b}}{\Delta_{-b}}\leq 16c_1^2 \frac{n_b}{n_{-b}}.
		\\&\red{\frac{\max_{i\in\Tc_{b}}\ellp_{t,i}}{\min_{i\in\Tc_{-b}}\ellp_{t,i}} \leq 4c_1^2 \frac{\Delta_{-b}}{\Delta_{b}} \leq 16c_1^2 \frac{n_{-b}}{n_b}}
	\end{align*}
	Hence, it suffices that
	\begin{align*}
	&\frac{c_0-E }{1/2-c_0} \leq  \frac{1}{16c_1^2} \Leftarrow c_0 \leq \frac{1/2-16c_1^3/C+16c_1^2(R_-/R_+)}{1+16c_1^2}.\\
	&\red{c_0 \leq \min \{\frac{1}{2}, \frac{8c_1^2+R_-/R_+-c_1/C}{1+16c_1^2} \}.}
	\end{align*}
	Provided that $R_-/R_+\geq0$ and since $C$ can be set large enough (say relative to $c_1$), we can always choose positive $c_0$ satisfying the above.
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%--------------------------- THEOREM 1 -------------------------------------
\tina{Have we defined $R_wst^\infty$}


Now we are ready to prove Theorem \ref{thm:main}. We start from Lemma \ref{lem:wsterror},
\begin{align*}
	\Rc_{wst, \rm{VS}}^\infty &= Q\big(\min_{b\in\{\pm 1\}}\inp{\nicefrac{\w^\infty}{\|\w^\infty\|_2}}{{\nub_{b}}}\big)\\
	&\leq Q\big(\inp{\nicefrac{\w^\infty}{\|\w^\infty\|_2}}{{\nub_{b}}}\big) \\
	&=Q\big(\lim_{t\to\infty}\inp{\nicefrac{\w^t}{\|\w^t\|_2}}{{\nub_{b}}}\big) \quad b \in \{\pm1\}
\end{align*}
To bound the worst-group error, it suffices to find an upper bound for $\rho_{t,b} = \inp{\w^t}{\nub_{b}}$ and a lower bound on  $\|\w^t\|_2$. Based on Lemma \ref{lem:corrLB}, we have,
\begin{align*}
	\inp{\nicefrac{\w^t}{\|\w^t\|_2}}{{\nub_{b}}} &= \frac{\rho_{t,b}}{\|\w^t\|_2}\\
	& \geq \frac{\rho_{0,b}+ {\eta\, R_+}\, \left( \frac{1}{2} \Lpall + 
		\Big(\frac{R_-}{R_+} -  \frac{c_1}{C}\Big)\Lpallneg\right)}{\|{\w^{0}}\|_2 + \eta \, c_1\,\sqrt{d}\,\Lpalls}\\
	&\geq \frac{\rho_{0,b}+ {\eta\,c_0\, R_+\,\Lpalls}\,}{\|{\w^{0}}\|_2 + \eta \, c_1\,\sqrt{d}\,\Lpalls}
\end{align*} 
where in the last line we used the Lemma \ref{lem:comparison}. Based on ??? we know that $\|\w^t\|\to \infty$. Since $\|\w^t\|$ is bounded by \ref{eq:normUB}, $L^\prime_{0:\infty} \to \infty$. Thus we have,
\begin{align*}
	\lim_{t\to\infty}\inp{\nicefrac{\w^t}{\|\w^t\|_2}}{{\nub_{b}}} &\geq \lim_{t\to\infty} \frac{\rho_{0,b}+ {\eta\,c_0\, R_+\,\Lpalls}\,}{\|{\w^{0}}\|_2 + \eta \, c_1\,\sqrt{d}\,\Lpalls} \\
	&= c\frac{R_+}{\sqrt{d}}
\end{align*}
And finally, since Q-function is decreasing,
\begin{align*}
	\Rc_{wst, \rm{VS}}^\infty &\leq Q\big( c {R_+}\big/{\sqrt{d}}\big)\, .
\end{align*}

%%--------------------------- THEOREM 2 -------------------------------------
\subsection{Putting things together: Proof of Theorem \ref{thm:LALoss}}
Similar to previous section, we start be the definition of worst group error,
\begin{align*}
	\Rc_{wst, \rm{LS}}^\infty &= Q\big(\min_{b\in\{\pm 1\}}\inp{\nicefrac{\w^\infty}{\|\w^\infty\|_2}}{{\nub_{b}}}\big)\\
	&= \max_{b \in \{\pm 1\}} Q\big(\inp{\nicefrac{\w^\infty}{\|\w^\infty\|_2}}{{\nub_{b}}}\big)
\end{align*}
We will provide a lower bound on the value of the objective function for the minority group (i.e. $b=-1$), which will also bound the $\Rc_{wst, \rm{LS}}^\infty$ from below.
From Lemma ???, for $t>t_0$,
\begin{align*}
	\inp{\nicefrac{\w^t}{\|\w^t\|_2}}{{\nub_{b}}} &= \frac{\rho_{t,b}}{\|\w^t\|_2}\\
	& \leq \frac{\rho_{t_0,b} +\eta R_+\left(\frac{3}{2}L^\prime_{t_0:t,b} + \Big(\frac{R_-}{R_+}+\frac{c_1}{C}\Big)L^\prime_{t_0:t,-b}\right)}{\|\w^{t_0}\|_2 + \frac{\eta c_2}{4} \, \sqrt{\frac{d}{n}} L^\prime_{t_0:t}}\\
	& \leq \frac{\rho_{t_0,b} +\eta R_+\left(\frac{3}{2}\frac{c_3 \, n_b}{n} + \Big(\frac{R_-}{R_+}+\frac{c_1}{C}\Big) \frac{c_3 \, n_{-b}}{n}\right)L^\prime_{t_0:t}}{\|\w^{t_0}\|_2 + \frac{\eta c_2}{4} \, \sqrt{\frac{d}{n}} L^\prime_{t_0:t}}
\end{align*}
\tina{killing log(n/delta)??}

Putting \eqref{eq:corrtheorem2} and \eqref{eq:normtheorem2} together for $t>t_0$,
\begin{align*}
\frac{\rho_{t,b}}{\|\w^t\|_2} &\leq \frac{\rho_{t_0,b} + \eta c' R_+ \big(\frac{n_b}{n_{-b}} + \frac{R_-}{R_+} + c_1\sqrt{\frac{\log(n/\delta)}{R_+}}\big) L^\prime_{t_0:t}}{\|\w^{t_0}\|_2+\eta c''\sqrt{\frac{d}{n}} L^\prime_{t_0:t}}
%&= c\sqrt{\frac{n}{d}}R_+(\frac{R_-}{R_+} + \frac{n_b}{n_{-b}}).	
\end{align*}
From GD step and \eqref{eq:z_norm}, we have $\norm{\w^t}_2 \leq \norm{\w^{t_0}}_2 + \eta L^\prime_{t_0:t} $. Since $\norm{\w^t}_2$ is unbounded, we can conclude that $L^\prime_{t_0:t} \rightarrow \infty$ as $t$ gets large. Hence, the second term containing $L^\prime_{t_0:t}$ will dominate and for large $t$,
\begin{align}
\lim_{t\to\infty} \frac{\inp{\w^t}{\nub_{b}}}{\|\w^t\|_2} &\leq cR_+\sqrt{\frac{n}{d}}\Big( \frac{n_b}{n_{-b}} + \frac{R_-}{R_+} + c_1\sqrt{\frac{\log(n/\delta)}{R_+}} \Big).
\end{align}
For $b=-1$ Thus, the term above is minimized when $b=-1$. Finally, the worst-group error can be bounded as follows.
\begin{align*}
\Rc_{wst, \rm{LA}}^\infty &\geq Q\big(\inp{\nicefrac{\w^\infty}{\|\w^\infty\|_2}}{{\nub_{-1}}}\big)\\
&\geq Q\Bigg(c\,R_+\,\sqrt{\frac{n}{d}}\,\Big(\frac{1}{\tau} + \frac{R_-}{R_+}+ 
{c_1\sqrt{\frac{\log(n/\delta)}{R_+}}} \Big)\Bigg).
\end{align*}

